Model Failure or Data Corruption? Exploring Inconsistencies in Building Energy Ratings with Self-Supervised Contrastive Learning

Building Energy Rating (BER) stands as a pivotal metric, enabling building owners, policymakers, and urban planners to understand the energy-saving potential through improving building energy efficiency. As such, enhancing buildings' BER levels is expected to directly contribute to the reduction of carbon emissions and promote climate improvement. Nonetheless, the BER assessment process is vulnerable to missing and inaccurate measurements. In this study, we introduce \texttt{CLEAR}, a data-driven approach designed to scrutinize the inconsistencies in BER assessments through self-supervised contrastive learning. We validated the effectiveness of \texttt{CLEAR} using a dataset representing Irish building stocks. Our experiments uncovered evidence of inconsistent BER assessments, highlighting measurement data corruption within this real-world dataset.

==> figures/boxplot.tex <==

\begin{figure}[th!]
\captionsetup{justification=centering}
         \centering
         \includegraphics[width=0.48\textwidth, 
         height=4cm
         ,trim={0cm 1cm 0cm 3cm},clip
         ]
        {figures/boxplot}
         \caption{five categories}
  
\end{figure}





==> sections/tables/ber_ml.tex <==
\begin{table}[htb]
\centering
\csvreader[
% no head,
% head to column names,
    head=False,
    before reading=\footnotesize
    % \sisetup{round-mode=places,round-precision=2,round-integer-to-decimal}
        \caption{Comparison of different BER granuairity classification with machine learning methods}\label{tab:algebraI}
          \setlength{\tabcolsep}{2.5pt},
    % tabular={c | S l | S c | c | c},
%     p{'width'}	paragraph column with text vertically aligned at the top
% m{'width'}	paragraph column with text vertically aligned in the middle (requires array package)
% b{'width'}	paragraph column with text vertically aligned at the bottom (requires array package)
        tabular={|>{\centering\arraybackslash}m{0.15\linewidth}
        |>{\centering\arraybackslash}m{0.15\linewidth} 
        |>{\centering\arraybackslash}m{0.25\linewidth} 
        |>{\centering\arraybackslash}m{0.15\linewidth} 
        % |>{\centering\arraybackslash}m{0.18\linewidth} 
        |
        },
    table head =\hline col1 & \# col2
    & \#  col3
    & \# col4 \\\hline\hline,
    late after line= \\,
    late after last line=\\\hline
    % \multicolumn{7}{c}{Total Score: 148}
    ]{sections/tables/test.csv}{}
{\csvcoli & \csvcolii & \csvcoliii & \csvcoliv}
% {\csvcoli & \csvcoliii}
\label{tab:ber}
\end{table}


==> sections/tables/ml_table.tex <==
% \begin{table}[h!]
% \centering
% \begin{tabular}{c|c|c|c}
\begin{tabular}{ | m{5em} | m{6em}| m{3em} | m{2em} | } 
\hline
% Classification & Performance Measure & Random Forest & MLP \\ \hline
% \multirow{2}{*}{A1, A2, ..., E, F, G} & Accuracy (\%) & 62.8 & \textbf{69.5} \\ 
%                      & Macro F1 (\%) & 63.1 & \textbf{63.9} \\ \hline
% \multirow{2}{*}{A, B, C, D, EFG}      & Accuracy (\%) & 76.1 & \textbf{88.6} \\ 
%                      & Macro F1 (\%) & 75.8 & \textbf{88.9} \\ \hline
% \end{tabular}
BER Levels & {Performance \newline Measure} & Random \newline Forest & MLP \\ \hline
\multirow{2}{*}{\shortstack{A1, A2, ..., \\ E, F, G}} & Accuracy (\%) & 62.8 & \textbf{69.5} \\  & Macro F1 (\%) & 63.1 & \textbf{63.9} \\ \hline
\multirow{2}{*}{\shortstack{A, B, C, D, \\EFG}}      & Accuracy (\%) & 76.1 & \textbf{88.6} \\ 
                     & Macro F1 (\%) & 75.8 & \textbf{88.9} \\ \hline
\end{tabular}
% \caption{ Comparison of different BER granularity classification with machine learning methods.}
% \label{table:comparison}
% \end{table}

==> sections/tables/table_and_boxplot.tex <==
  \begin{minipage}{\textwidth}
  \begin{minipage}[b]{0.5\textwidth}
% \captionsetup{justification=centering}
\input{sections/tables/ml_table}
    \captionof{table}{ Performance Comparison of Machine Learning Models for BER Prediction with Different Level Granularity}
\label{table:comparison}
  \end{minipage}
  \hfill
\begin{minipage}[b]{0.45\textwidth}
    \captionsetup{justification=centering}
         \centering
         \includegraphics[width=\textwidth, 
         height=3cm
         ,trim={0cm 1cm 0cm 5cm},clip
         ]
        {figures/boxplot.jpeg}
         \captionof{figure}{Box-plot}
         \end{minipage}
\end{minipage}  
